A Unifying Review of Deep and Shallow Anomaly Detection

Deep learning approaches to anomaly detection have recently improved the state of the art in detection performance on complex datasets such as large collections of images or text. These results have sparked a renewed interest in the anomaly detection problem and led to the introduction of a great variety of new methods. With the emergence of numerous such methods, including approaches based on generative models, one-class classification, and reconstruction, there is a growing need to bring methods of this field into a systematic and unified perspective. In this review we aim to identify the common underlying principles as well as the assumptions that are often made implicitly by various methods. In particular, we draw connections between classic 'shallow' and novel deep approaches and show how this relation might cross-fertilize or extend both directions. We further provide an empirical assessment of major existing methods that is enriched by the use of recent explainability techniques, and present specific worked-through examples together with practical advice. Finally, we outline critical open challenges and identify specific paths for future research in anomaly detection.

==> A Unifying Review of Anomaly Detection/appx.tex <==
\section{Notation and Abbreviations}

For reference, we provide the notation and abbreviations used in this work in Tables \ref{tab:notation} and \ref{tab:abbrev} respectively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
    \caption{Notation Conventions}
    \label{tab:notation}
    \centering
    \input{tab/notation}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
    \caption{List of Abbreviations}
    \label{tab:abbrev}
    \centering
    \input{tab/abbrev}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Additional Details on Experimental Evaluation}
\label{appendix:exp_details}

\subsection{Average Precision on MNIST-C and MVTec-AD}
\label{appendix:avg_precision}

We provide the detection performance measured in Average Precision (AP) of the experimental evaluation on MNIST-C and MVTec-AD from section \ref{ssec:comparison} in Tables \ref{tab:mnist-c_ap} and \ref{tab:mvtec_ap} respectively.
As can be seen (and as to be expected \cite{davis2006}), the performance in AP here shows the same trends as AUC (cf., Tables \ref{tab:mnist-c_auc} and \ref{tab:mvtec_auc} in section \ref{ssec:comparison}), since the MNIST-C and MVTec-AD test sets are not highly imbalanced.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[th]
    \caption{AP detection performance on MNIST-C.}
    \label{tab:mnist-c_ap}
    \centering
    \resizebox{\columnwidth}{!}{\input{tab/mnist-c_ap}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
    \caption{AP detection performance on MVTec-AD.}
    \label{tab:mvtec_ap}
    \centering
    \resizebox{\columnwidth}{!}{\input{tab/mvtec_ap}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Training Details}
\label{appendix:training_details}

For PCA, we compute the reconstruction error whilst maintaining 90\% of variance of the training data. 
We do the same for kPCA, and additionally choose the kernel width such that 50\% neighbors capture 50\% of total similarity scores.
For MVE, we use the fast minimum covariance determinant estimator \cite{rousseeuw1999} with a default support fraction of 0.9 and a contamination rate parameter of 0.01.
To facilitate MVE computation on MVTec-AD, we first reduce the dimensionality via PCA retaining 90\% of variance.
For KDE, we choose the bandwidth parameter to maximize the likelihood of a small hold-out set from the training data.
For SVDD, we consider $\nu \in \{0.01, 0.05, 0.1, 0.2\}$ and select the kernel scale using a small labeled hold-out set.
The deep one-class classifier applies a whitening transform on the representations after the first fully-connected layer of a pre-trained VGG16 model (on MVTec-AD) or a CNN classifier trained on the EMNIST letter subset (on MNIST-C).
For the AE on MNIST-C, we use a LeNet-type encoder that has two convolutional layers with max-pooling followed by two fully connected layers that map to an encoding of 64 dimensions, and construct the decoder symmetrically.
On MVTec-AD, we use an encoder-decoder architecture as presented in \cite{huang2019} which maps to a bottleneck of 512 dimensions. Both, the encoder and decoder here consist of four blocks having two 3${\times}$3 convolutional layers followed by max-pooling or upsampling respectively. 
We train the AE such that the reconstruction error of a small training hold-out set is minimized.
For AGAN, we use the AE encoder and decoder architecture for the discriminator and generator networks respectively, where we train the GAN until convergence to a stable equilibrium.


\subsection{Explaining KDE}
\label{appendix:xai}
The model can be neuralized as described in Section \ref{ssec:xai}, replacing the squared Euclidean distance in the first layer with a squared Mahalanobis distance. The heatmaps of both models (KDE and Mahalanobis KDE) are computed as
\[
R = \tfrac12\sum_{j=1}^n (\bx_j - \bx) \odot \nabla_{\bx_j}s(\bx),
\]
where $\odot$ denotes element-wise multiplication.
This implements a Taylor-type decomposition as described in \cite{kauffmann2020}.


\subsection{Open Source Software, Tutorials, and Demos}
For the implementation of the shallow MVE and SVDD models, we have used the \texttt{scikit-learn} library \cite{scikit-learn} available at \url{https://scikit-learn.org/}.
For the implementation of the shallow Gauss, PCA, KDE, and kPCA models as well as the deep AGAN, DOCC, RealNVP, and AE models, we have used the \texttt{PyTorch} library \cite{pytorch} available at \url{https://pytorch.org/}.
Implementations of the Deep SVDD and Deep SAD methods are available at \url{https://github.com/lukasruff/}.
Tutorials, demos, and code for explainable AI techniques, in particular LRP, can be found at \url{http://www.heatmapping.org/}.
In the spirit of \emph{the need for open source software in machine learning} \cite{sonnenburg2007}, a similar collection of tutorials, demos, and code on anomaly detection methods are in the making and will be made available at \url{http://www.pyano.org/}.



==> A Unifying Review of Anomaly Detection/tab/abbrev.tex <==
\begin{tabular}{ll}
    \toprule
    Abbreviation        & Description \\
    \midrule
    AD      & Anomaly Detection \\
    AE		& Autoencoder \\
    AP		& Average Precision \\
    AAE		& Adversarial Autoencoder \\
    AUPRC   & Area Under the Precision-Recall Curve \\
    AUROC	& Area Under the ROC curve \\
    CAE		& Contrastive Autoencoder \\
    DAE		& Denoising Autoencoder \\
    DGM		& Deep Generative Model \\
    DSVDD	& Deep Support Vector Data Description \\
    DSAD	& Deep Semi-supervised Anomaly Detection \\
    EBM		& Energy Based Model \\
    ELBO	& Evidence Lower Bound \\
    GAN		& Generative Adversarial Network \\
    GMM		& Gaussian Mixture Model \\
    GT		& Geometric Transformations \\
    iForest & Isolation Forest \\
    KDE		& Kernel Density Estimation \\
    $k$-NN	& $k$-Nearest Neighbors \\
    kPCA	& Kernel Principal Component Analysis \\
    LOF		& Local Outlier Factor \\
    LPUE	& Learning from Positive and Unlabeled Examples \\
    LSTM	& Long short-term memory \\
    MCMC	& Markov chain Monte Carlo \\
    MCD		& Minimum Covariance Determinant \\
    MVE		& Minimum Volume Ellipsoid \\
    OOD		& Out-of-distribution \\
    OE		& Outlier Exposure \\
    OC-NN	& One-Class Neural Network \\
    OC-SVM	& One-Class Support Vector Machine \\
    pPCA	& Probabilistic Principal Component Analysis \\
    PCA		& Principal Component Analysis \\
    pdf		& Probability density function \\
    PSD		& Positive semidefinite \\
    RBF		& Radial basis function \\
    RKHS	& Reproducing Kernel Hilbert Space \\
    rPCA	& Robust Principal Component Analysis \\
    SGD		& Stochastic Gradient Descent \\
    SGLD	& Stochastic Gradient Langevin Dynamics \\
    SSAD	& Semi-Supervised Anomaly Detection \\
    SVDD	& Support Vector Data Description \\
    VAE		& Variational Autoencoder \\
    VQ		& Vector Quantization \\
    XAI		& Explainable AI \\
    \bottomrule
\end{tabular}


==> A Unifying Review of Anomaly Detection/tab/benchmarks.tex <==
\begin{tabular}{rl}
    \toprule
    {\bf $k$-classes-out} & \parbox{.7\linewidth}{(Fashion-)MNIST, CIFAR-10, STL-10, ImageNet}\\\midrule
    {\bf Synthetic} & \parbox{.7\linewidth}{MNIST-C \cite{mnist-c}, ImageNet-C \cite{hendrycks2019b}, ImageNet-P \cite{hendrycks2019b}, ImageNet-O \cite{hendrycks2019e}} \\\midrule
    {\bf Real-world} & \parbox{.7\linewidth}{{\em Industrial:} MVTec-AD \cite{bergmann2019}, PCB \cite{huang2019pcb}\\
    {\em Medical:} CAMELYON16 \cite{bejnordi2017,tuluptceva2020}, NIH Chest X-ray \cite{Wang_2017,tuluptceva2020}, MOOD \cite{mood}, HCP/BRATS \cite{chen2018}, Neuropathology \cite{faust2018,naud2020}\\
    {\em Security:} Credit-card-fraud \cite{pozzolo2018}, URL \cite{ma2009}, UNSW-NB15 \cite{moustafa2015}\\
    {\em Time series:} NAB \cite{ahmad2017}, Yahoo \cite{laptev2015}\\
    {\em Misc.:} Emmott \cite{Emmott2016}, ELKI \cite{campos2016}, ODDS \cite{rayana2016}, UCI \cite{domingues2018,Dua:2019}}\\
    \bottomrule
\end{tabular}

==> A Unifying Review of Anomaly Detection/tab/data_properties.tex <==
\begin{tabular}{ll}
    \toprule
    Data Property               & Description \\
    \midrule
    Size $n+m$                  & \parbox[t][][t]{6.2cm}{Is algorithm scalability in dataset size critical? Are there labeled samples ($m>0$) for (semi-)supervision?} \\[12pt]
    Dimension $D$               & \parbox[t][][t]{6.2cm}{Low- or high-dimensional? Truly high-dimensional or embedded in some higher dimensional ambient space?} \\[12pt]
    Type                        & \parbox[t][][t]{6.2cm}{Continuous, discrete, or categorical?} \\[2pt]
    Scales                      & \parbox[t][][t]{6.2cm}{Are features uni- or multi-scale?} \\[2pt]
    Modality                    & \parbox[t][][t]{6.2cm}{Uni- or multimodal (classes and clusters)? Is there a hierarchy of sub- and superclasses (or -clusters)?} \\[12pt]
    Convexity                   & \parbox[t][][t]{6.2cm}{Is the data support convex or non-convex?} \\[2pt]
    Correlation                 & \parbox[t][][t]{6.2cm}{Are features (linearly or non-linearly) correlated?} \\[2pt]
    Manifold                    & \parbox[t][][t]{6.2cm}{Has the data a (linear, locally linear, or non-linear) subspace or manifold structure? Are there invariances (translation, rotation, etc.)?} \\[21pt]
    Hierarchy                   & \parbox[t][][t]{6.2cm}{Is there a natural feature hierarchy (e.g., images, video, text, speech, etc.)? Are low-level or high-level (semantic) anomalies relevant?} \\[21pt]
    Context                     & \parbox[t][][t]{6.2cm}{Are there contextual features (e.g., time, space, sequence, graph, etc.)? Can anomalies be contextual?} \\[12pt]
    Stationarity                & \parbox[t][][t]{6.2cm}{Is the distribution stationary or non-stationary? Is a domain or covariate shift expected?}\\[12pt]
    Noise                       & \parbox[t][][t]{6.2cm}{Is the noise level $\varepsilon$ large or small? Is the noise type Gaussian or more complex?}\\[12pt]
    Contamination               & \parbox[t][][t]{6.2cm}{Is the data contaminated with anomalies? What is the contamination rate $\eta$?}\\
    \bottomrule
\end{tabular}


==> A Unifying Review of Anomaly Detection/tab/mnist-c_ap.tex <==
\begin{tabular}{rccccccccc}\toprule
& Gaussian & MVE & PCA & KDE & SVDD & kPCA & AGAN & DOCC & AE\\\midrule
          brightness & \bf 100.0 &      98.0 & \bf 100.0 & \bf 100.0 &     100.0 & \bf 100.0 & \bf 100.0 &      32.9 & \bf 100.0\\
         canny edges &      99.1 &      58.8 & \bf 100.0 &      71.8 &      96.6 &      99.9 &     100.0 &      97.7 &     100.0\\
         dotted line &      99.9 &      56.8 &      99.0 &      63.4 &      67.9 &      90.9 &      88.8 &      81.5 & \bf  99.9\\
                 fog &     100.0 &      88.3 &      98.7 &      75.5 &      94.2 &      94.2 & \bf 100.0 &      34.8 &     100.0\\
          glass blur &      78.6 &      42.0 &      65.5 &      31.5 &      45.9 &      36.2 & \bf 100.0 &      37.6 &      99.6\\
       impulse noise & \bf 100.0 &      59.8 & \bf 100.0 &      97.1 &      99.6 & \bf 100.0 & \bf 100.0 &      96.2 & \bf 100.0\\
         motion blur &      52.6 &      44.3 &      37.3 &      31.5 &      47.1 &      33.9 & \bf 100.0 &      66.5 &      93.8\\
              rotate &      44.1 &      52.2 &      38.3 &      42.3 &      56.3 &      43.5 & \bf  93.6 &      66.0 &      53.1\\
               scale &      31.9 &      34.5 &      33.0 &      31.2 &      39.4 &      34.4 &      61.9 & \bf  70.2 &      42.5\\
               shear &      72.7 &      62.0 &      64.2 &      52.5 &      59.0 &      60.0 & \bf  95.5 &      66.5 &      70.4\\
          shot noise &      93.6 &      44.8 &      97.3 &      42.7 &      60.4 &      81.7 &      96.8 &      49.0 & \bf  99.7\\
             spatter & \bf  99.8 &      50.5 &      82.6 &      45.8 &      54.8 &      61.2 &      99.2 &      63.2 &      97.1\\
              stripe & \bf 100.0 &      99.9 & \bf 100.0 & \bf 100.0 &     100.0 & \bf 100.0 & \bf 100.0 &     100.0 & \bf 100.0\\
           translate &      95.5 &      64.8 &      97.0 &      73.7 &      92.2 &      95.7 &      97.2 & \bf  98.6 &      93.7\\
              zigzag &      99.8 &      64.6 &     100.0 &      79.4 &      86.5 &      99.3 &      98.0 &      94.8 & \bf 100.0\\
\bottomrule\end{tabular}


==> A Unifying Review of Anomaly Detection/tab/mnist-c_auc.tex <==
\begin{tabular}{rccccccccc}\toprule
& Gaussian & MVE & PCA & KDE & SVDD & kPCA & AGAN & DOCC & AE\\\midrule
          brightness & \bf 100.0 &      99.0 & \bf 100.0 & \bf 100.0 &     100.0 & \bf 100.0 & \bf 100.0 &      13.7 & \bf 100.0\\
         canny edges &      99.4 &      68.4 & \bf 100.0 &      78.9 &      96.3 &      99.9 &     100.0 &      97.9 &     100.0\\
         dotted line &      99.9 &      62.9 &      99.3 &      68.5 &      70.0 &      92.6 &      91.5 &      86.4 & \bf 100.0\\
                 fog &     100.0 &      89.6 &      98.1 &      62.1 &      92.3 &      91.3 & \bf 100.0 &      17.4 &     100.0\\
          glass blur &      79.5 &      34.7 &      70.7 &       8.0 &      49.1 &      27.1 & \bf 100.0 &      31.1 &      99.6\\
       impulse noise & \bf 100.0 &      69.0 & \bf 100.0 &      98.0 &      99.7 & \bf 100.0 & \bf 100.0 &      97.5 & \bf 100.0\\
         motion blur &      38.1 &      43.4 &      24.3 &       8.1 &      50.2 &      18.3 & \bf 100.0 &      70.7 &      95.1\\
              rotate &      31.3 &      54.7 &      24.9 &      37.1 &      57.7 &      38.7 & \bf  93.2 &      65.5 &      53.4\\
               scale &       7.5 &      20.7 &      14.5 &       5.0 &      36.5 &      19.6 &      68.1 & \bf  79.8 &      40.4\\
               shear &      63.7 &      58.1 &      55.5 &      49.9 &      58.2 &      54.1 & \bf  94.9 &      64.6 &      70.6\\
          shot noise &      94.9 &      43.2 &      97.1 &      41.6 &      63.4 &      81.5 &      96.7 &      51.5 & \bf  99.7\\
             spatter & \bf  99.8 &      52.6 &      85.0 &      44.5 &      57.3 &      64.5 &      99.0 &      68.2 &      97.4\\
              stripe & \bf 100.0 &      99.9 & \bf 100.0 & \bf 100.0 &     100.0 & \bf 100.0 & \bf 100.0 &     100.0 & \bf 100.0\\
           translate &      94.5 &      73.9 &      96.3 &      76.2 &      91.8 &      94.8 &      97.3 & \bf  98.8 &      92.2\\
              zigzag &      99.9 &      72.5 &     100.0 &      84.0 &      87.7 &      99.4 &      98.3 &      94.3 & \bf 100.0\\
\bottomrule\end{tabular}


==> A Unifying Review of Anomaly Detection/tab/mvtec_ap.tex <==
\begin{tabular}{rrccccccccc}\toprule
& & Gaussian & MVE & PCA & KDE & SVDD & kPCA & AGAN & DOCC & AE\\\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{Textures}}
&      carpet &      77.3 &      86.9 &      71.0 &      70.2 &      77.4 &      69.8 &      94.3 & \bf  97.2 &      70.9\\
&        grid &      79.9 &      80.8 &      91.7 &      85.5 &      89.2 &      88.7 & \bf  97.4 &      75.4 &      84.8\\
&     leather &      72.9 &      81.1 &      85.8 &      75.3 &      83.6 &      86.3 &      82.1 & \bf  92.3 &      87.7\\
&        tile &      84.4 &      91.6 &      80.5 &      85.1 &      86.9 &      83.9 &      88.8 & \bf  98.6 &      78.1\\
&        wood &      82.0 &      93.8 &      97.0 & \bf  98.5 &      98.3 &      97.1 &      92.0 &      97.6 &      96.8\\\midrule
\multirow{10}{*}{\rotatebox[origin=c]{90}{Objects}}
&      bottle &      92.3 &      86.2 &      99.2 &      94.2 &      96.7 &      98.9 &      97.2 & \bf  99.9 &      98.5\\
&       cable &      73.2 &      76.6 &      85.9 &      78.5 &      82.9 &      84.2 &      81.2 & \bf  94.1 &      71.3\\
&     capsule &      92.3 &      89.3 &      93.0 &      85.9 &      88.7 &      92.0 &      84.3 & \bf  97.9 &      82.8\\
&    hazelnut &      81.9 &      89.3 &      94.2 &      83.2 &      85.7 &      90.9 & \bf  98.1 &      97.5 &      95.0\\
&   metal nut &      86.3 &      82.6 &      86.5 &      75.0 &      86.0 &      87.4 &      92.7 & \bf  96.3 &      77.0\\
&        pill &      91.8 &      93.8 & \bf  96.5 &      91.7 &      95.0 &      96.1 &      90.6 &      95.6 &      94.5\\
&       screw &      78.0 &      71.4 &      86.6 &      69.1 &      55.4 &      77.0 & \bf  99.8 &      95.1 &      90.3\\
&  toothbrush &      97.6 &      87.6 & \bf  99.4 &      97.4 &      98.5 & \bf  99.4 &      86.9 &      98.7 &      73.9\\
&  transistor &      70.5 &      54.7 &      80.7 &      70.1 &      74.1 &      79.7 &      71.2 & \bf  90.0 &      51.4\\
&      zipper &      81.0 &      84.2 &      91.8 &      82.8 &      87.9 &      91.5 &      85.7 & \bf  97.8 &      79.3\\
\bottomrule\end{tabular}


==> A Unifying Review of Anomaly Detection/tab/mvtec_auc.tex <==
\begin{tabular}{rrccccccccc}\toprule
& & Gaussian & MVE & PCA & KDE & SVDD & kPCA & AGAN & DOCC & AE\\\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{Textures}}
&      carpet &      48.8 &      63.5 &      45.6 &      34.8 &      48.7 &      41.9 &      83.1 & \bf  90.6 &      36.8\\
&        grid &      60.6 &      67.8 &      81.8 &      71.7 &      80.4 &      76.7 & \bf  91.7 &      52.4 &      74.6\\
&     leather &      39.6 &      49.5 &      60.3 &      41.5 &      57.3 &      61.1 &      58.6 & \bf  78.3 &      64.0\\
&        tile &      68.5 &      79.7 &      56.4 &      68.9 &      73.3 &      63.2 &      74.1 & \bf  96.5 &      51.8\\
&        wood &      54.0 &      80.1 &      90.4 & \bf  94.7 &      94.1 &      90.6 &      74.5 &      91.6 &      88.5\\\midrule
\multirow{10}{*}{\rotatebox[origin=c]{90}{Objects}}
&      bottle &      78.9 &      67.0 &      97.4 &      83.3 &      89.3 &      96.3 &      90.6 & \bf  99.6 &      95.0\\
&       cable &      56.5 &      71.9 &      77.6 &      66.9 &      73.1 &      75.6 &      69.7 & \bf  90.9 &      57.3\\
&     capsule &      71.6 &      65.1 &      75.7 &      56.2 &      61.3 &      71.5 &      60.7 & \bf  91.0 &      52.5\\
&    hazelnut &      67.6 &      80.4 &      89.1 &      69.9 &      74.3 &      83.8 & \bf  96.4 &      95.0 &      90.5\\
&   metal nut &      54.7 &      45.1 &      56.4 &      33.3 &      54.3 &      59.0 &      79.3 & \bf  85.2 &      45.5\\
&        pill &      65.5 &      71.5 & \bf  82.5 &      69.1 &      76.2 &      80.7 &      64.6 &      80.4 &      76.0\\
&       screw &      53.5 &      35.5 &      67.9 &      36.9 &       8.6 &      46.7 & \bf  99.6 &      86.9 &      77.9\\
&  toothbrush &      93.9 &      76.1 & \bf  98.3 &      93.3 &      96.1 & \bf  98.3 &      70.8 &      96.4 &      49.4\\
&  transistor &      70.2 &      64.8 &      81.8 &      72.4 &      74.8 &      80.0 &      78.8 & \bf  90.8 &      51.2\\
&      zipper &      50.1 &      65.2 &      82.8 &      61.4 &      68.6 &      81.0 &      69.7 & \bf  92.4 &      35.0\\
\bottomrule\end{tabular}


==> A Unifying Review of Anomaly Detection/tab/notation.tex <==
\begin{tabular}{ll}
    \toprule
    Symbol                  & Description \\
    \midrule
    $\bbN$                  & The natural numbers \\
    $\bbR$                  & The real numbers \\
    $D$                     & The input data dimensionality $D \in \bbN$ \\
    $\calX$                 & The input data space $\calX \subseteq \bbR^D$ \\
    $\calY$                 & The labels $\calY = \{\pm 1\}$ (${+1}$ : normal; ${-1}$ : anomaly) \\
    $\bx$                   & A vector, e.g.\ a data point $\bx \in \calX$ \\
    $\calD_n$               & An unlabeled dataset $\calD_n = \{ \bx_1, \ldots, \bx_n \}$ of size $n$ \\
    $\Pgen, \pgen$          & The data-generating distribution and pdf \\
    $\Pnorm, \pnorm$        & The normal data distribution and pdf \\
    $\Pout, \pout$          & The anomaly distribution and pdf \\
    $\phat$                 & An estimated pdf \\
    $\varepsilon$           & An error or noise distribution\\
    $\supp(p)$              & \makecell[tl]{The support of a data distribution $\mathbb{P}$ with density $p$,\\ i.e.\ $\{ \bx \in \mathcal{X} \, | \, p(\bx) > 0 \}$} \\
    $\calA$                 & The set of anomalies \\
    $C_\alpha$              & An $\alpha$-density level set \\
    $\hat{C}_\alpha$        & An $\alpha$-density level set estimator \\
    $\tau_\alpha$           & The threshold $\tau_\alpha \geq 0$ corresponding to $C_\alpha$ \\
    $c_\alpha(\bx)$         & The threshold anomaly detector corresponding to $C_\alpha$ \\
    $s(\bx)$                & An anomaly score function $s: \calX \to \bbR$ \\
    $\bbInd_{A}(\bx)$       & The indicator function for some set $A$ \\
    $\ell(s,y)$             & A loss function $\ell : \bbR \times \{\pm 1 \} \to \bbR$ \\
    $f_\theta(\bx)$         & A model $f_\theta : \calX \to \bbR$ with parameters $\theta$ \\
    $k(\bx, \tilde{\bx})$   & A kernel $k: \calX \times \calX \to \bbR$ \\
    $\calF_k$               & The RKHS or feature space of kernel $k$ \\
    $\phi_k(\bx)$           & The feature map $\phi_k : \calX \to \calF_k$ of kernel $k$ \\
    $\phi_\omega(\bx)$      & A neural network $\bx \mapsto \phi_\omega(\bx)$ with weights $\omega$ \\
    \bottomrule
\end{tabular}


==> A Unifying Review of Anomaly Detection/tab/taxonomy_methods.tex <==
\begin{tabular}{llllllllc}
    \toprule
    Method                  & Loss $\ell(s, y)$     & Model $f_\theta(\bx)$                                             & \multicolumn{2}{l}{Feature Map $\phi(\bx)$}   & Parameter $\theta$    & Regularization $\calR(f, \phi, \theta)$                                   & Bayes?        & References \\
    \midrule
    Parametric Density      & $-\log(s)$            & $p(\bx | \theta)$                                                 & $\bx$ & (input)                               & $\theta$              & choice of density class $\{p_{\theta} \, | \, \theta \in \Theta\}$        & \xmark & \cite{bishop2006,murphy2012} \\[1.5pt]
    Gaussian/Mahalanobis    & $-\log(s)$            & $\calN(\bx | \bmu, \Sigma)$                                       & $\bx$ & (input)                               & $(\bmu, \Sigma)$      & --                                                                        & \xmark & \cite{bishop2006,murphy2012} \\[1.5pt]
    GMM                     & $-\log(s)$            & $\sum_k \pi_k \, \calN(\bx | \bmu_k, \Sigma_k)$                   & $\bx$ & (input)                               & $(\pi, \bmu, \Sigma)$ & number of mixture components $K$                                          & latent & \cite{theodoridis2020} \\[1.5pt]
    KDE                     & $-\log(s)$            & $\exp(-\Vert \phi_k(\bx) - \bmu \Vert^2)$                         & $\phi_k(\bx)$ & (kernel)                      & $\bmu$                & kernel hyperparameters (e.g., bandwidth $h$)                              & \xmark & \cite{roberts1994b,bishop1994} \\[1.5pt]
    EBMs                    & $-\log(s)$            & $\tfrac{1}{Z(\theta)} \exp(-E(\phi(\bx), \bz; \theta))$           &  $\phi(\bx)$  & (various)                     & $\theta$              & latent prior $p(\bz)$ & latent & \cite{lecun2006,zhai2016} \\[1.5pt]
    Normalizing Flows       & $-\log(s)$            & $p_{\bz}(\phi_{\omega}^{-1}(\bx)) \, |\det J_{\phi_{\omega}^{-1}}(\bx)|$ & $\phi_\omega(\bx)$ & (neural)                 & $\omega$            & base distribution $p_{\bz}(\bz)$; diffeomorphism architecture & \xmark & \cite{papamakarios19,nachman20} \\[1.5pt]
    GAN ($D$-based)         & $-\log(s)$ & $\sigma(\langle \bw,\psi_\omega(\bx)\rangle)$ & $\psi_\omega(\bx)$ & (neural) & $(\bw,\omega)$ & adversarial training & \xmark & \cite{schlegl2019,sabokrou2020} \\[1.5pt]
    \midrule
    Min.\ Vol.\ Sphere      & $\max(0, s)$          & $\Vert \bx - \bc \Vert^2 - R^2$                                   & $\bx$ & (input)                               & $(\bc, R)$            & $\nu R^2$                                                     & \xmark & \cite{tax2001} \\[1.5pt]
    Min.\ Vol.\ Ellipsoid   & $\max(0, s)$          & $(\bx - \bc)^\top \Sigma^{-1} (\bx - \bc) - R^2$                  & $\bx$ & (input)                               & $(\bc, R, \Sigma)$    & $\nu (\tfrac{1}{2} \Vert \Sigma \Vert_{\Fr}^2 + R^2)$          & \xmark & \cite{rousseeuw1999} \\[1.5pt]
    SVDD                    & $\max(0, s)$          & $\Vert \phi_k(\bx) - \bc \Vert^2 - R^2$                           & $\phi_k(\bx)$ & (kernel)                      & $(\bc, R)$            & $\nu R^2$                                                     & \xmark & \cite{tax2004} \\[1.5pt]
    Semi-Sup.\ SVDD         & $\max(0, ys)$         & $\Vert \phi_k(\bx) - \bc \Vert^2 - R^2$                           & $\phi_k(\bx)$ & (kernel)                      & $(\bc, R)$            & $\nu R^2$                                                     & \xmark & \cite{tax2004,gornitz2013} \\[1.5pt]
    Soft Deep SVDD          & $\max(0, s)$          & $\Vert \phi_\omega(\bx) - \bc \Vert^2 - R^2$                           & $\phi_\omega(\bx)$ & (neural)                      & $(\bc, R, \omega)$         & $\nu R^2$; weight decay; collapse reg.\ (various)  & \xmark & \cite{ruff2018} \\[1.5pt]
    OC Deep SVDD            & $s$                   & $\Vert \phi_\omega(\bx) - \bc \Vert^2$                                 & $\phi_\omega(\bx)$ & (neural)                      & $(\bc, \omega)$            & weight decay; collapse reg.\ (various)               & \xmark & \cite{ruff2018} \\[1.5pt]
    Deep SAD                & $s^y$                 & $\Vert \phi_\omega(\bx) - \bc \Vert^2$                                 & $\phi_\omega(\bx)$ & (neural)                      & $(\bc, \omega)$            & weight decay                                  & \xmark & \cite{ruff2020} \\[1.5pt]
    OC-SVM                  & $\max(0, s)$          & $\rho - \langle \bw, \phi_k(\bx) \rangle$                         & $\phi_k(\bx)$ & (kernel)                      & $(\bw, \rho)$         & $\nu (\tfrac{1}{2} \Vert \bw \Vert^2 - \rho)$                  & \xmark & \cite{scholkopf2001} \\[1.5pt]
    OC-NN                   & $\max(0, s)$          & $\rho - \langle \bw, \phi_\omega(\bx) \rangle$                         & $\phi_\omega(\bx)$ & (neural)                      & $(\bw, \rho, \omega)$      & $\nu (\tfrac{1}{2} \Vert \bw \Vert^2 - \rho)$; weight decay & \xmark & \cite{chalapathy2018b} \\[1.5pt]
    Bayesian DD             & $\max(0, s)$          & $\Vert \phi_k(\bx) - \bc \Vert^2 - R^2$                           & $\phi_k(\bx)$ & (kernel)                      & $(\bc, R)$            & $\bc=\sum_i\alpha_i\phi_k(\bx_i)$ with prior $\alpha\sim\mathcal N(\boldsymbol\mu,\Sigma)$ & fully & \cite{ghasemi2012} \\[1.5pt]
    GT                      & $-\log(s)$            & $\prod_k \sigma_k(\langle \bw, \phi_\omega(T_k(\bx))\rangle)$   & $\phi_\omega(\bx)$ & (neural)                 & $(\bw,\omega)$        & transformations $\calT = \{T_1, \ldots, T_K\}$ for self-labeling & \xmark & \cite{golan2018,hendrycks2019d} \\[1.5pt]
    GOAD (CE)               & $-\log(s)$            & $\prod_k \sigma_k(-\Vert \phi_\omega(T_k(\bx)) - \bc_k \Vert^2)$  & $\phi_\omega(\bx)$ & (neural)                 & $(\bc_1, \ldots, \bc_K, \omega)$        & transformations $\calT = \{T_1, \ldots, T_K\}$ for self-labeling & \xmark & \cite{bergman2020b} \\[1.5pt]
    BCE (supervised)        & $-y \log(s){-}\tfrac{1{-}y}{2}\log(1{-}s)$ & $\sigma(\langle \bw, \phi_\omega(\bx)\rangle)$                & $\phi_\omega(\bx)$ & (neural)                      & $(\bw,\omega)$             & weight decay & \xmark & \cite{ruff2020b} \\[1.5pt]
    BNN (supervised)        & $-y \log(s){-}\tfrac{1{-}y}{2}\log(1{-}s)$ & $\sigma(\langle \bw, \phi_\omega(\bx)\rangle)$                & $\phi_\omega(\bx)$ & (neural)                      & $(\bw,\omega)$             & prior $p(\bw,\omega)$ & fully & \cite{mackay1992,blundell2015} \\
    \midrule
    PCA                     & $s$                   & $\Vert \bx - W^\top W \bx \Vert_2^2$                                      & $\bx$ & (input)                       & $W$                         & $W W^\top = I$                                                & \xmark & \cite{hawkins1974} \\[1.5pt]
    Robust PCA              & $s$                   & $\Vert \bx - W^\top W \bx \Vert_1$                                        & $\bx$ & (input)                       & $W$                         & $W W^\top = I$                                                & \xmark & \cite{kwak2008} \\[1.5pt]
    Probabilistic PCA       & $-\log(s)$            & $\calN(\bx | \bm{0}, W^\top W + \sigma^2 I)$                                   & $\bx$ & (input)                       & $(W, \sigma^2)$           & linear latent Gauss model $\bx = W^\top \bz + \varepsilon$    & latent & \cite{tipping1999} \\[1.5pt]
    Bayesian PCA            & $-\log(s)$            & $\calN(\bx | \bm{0}, W^\top W + \sigma^2 I) \, p(W | \bm{\alpha})$                & $\bx$ & (input)                       & $(W, \sigma^2)$           & linear latent Gauss model with prior $p(W | \bm{\alpha})$     & fully & \cite{bishop1999} \\[1.5pt]
    Kernel PCA              & $s$                   & $\Vert \phi_k(\bx) - W^\top W \phi_k(\bx) \Vert^2$                        & $\phi_k(\bx)$ & (kernel)              & $W$                         & $W W^\top = I$                                                & \xmark & \cite{scholkopf1998,hoffmann2007} \\[1.5pt]
    Autoencoder             & $s$                   & $\Vert \bx - \phi_\omega(\bx) \Vert_2^2$                                       & $\phi_\omega(\bx)$ & (neural)              & $\omega$                         & advers.\ (AAE), contract.\ (CAE), denois.\ (DAE), etc.\                       & \xmark & \cite{zhou2017,kim2020} \\[1.5pt]
    VAE                     & $-\log(s)$            & $p_{\phi_\omega}(\bx | \bz) $                                                  & $\phi_\omega(\bx)$ & (neural)              & $\omega$                         & latent prior $p(\bz)$                                         & latent & \cite{an2015,kingma2019} \\[1.5pt]
    GAN ($G$-based)         & $-\log(s)$            & $p_{\phi_\omega}(\bx | \bz) $                                                  & $\phi_\omega(\bx)$ & (neural)              & $\omega$                         & adversarial training and latent prior $p(\bz)$                       & latent & \cite{schlegl2017,deecke2018} \\[1.5pt]
    $k$-means               & $s$                   & $\Vert \bx - \argmin_{\bc_k} \Vert \bx - \bc_k \Vert_2 \Vert_2^2$         & $\bx$ & (input)                       & $(\bc_1, \ldots, \bc_K)$  & number of prototypes $K$                                      & \xmark & \cite{jain2010,theodoridis2020} \\[1.5pt]
    $k$-medians             & $s$                   & $\Vert \bx - \argmin_{\bc_k} \Vert \bx - \bc_k \Vert_1 \Vert_1$           & $\bx$ & (input)                       & $(\bc_1, \ldots, \bc_K)$  & number of prototypes $K$                                      & \xmark & \cite{jain2010} \\[1.5pt]
    VQ                      & $s$                   & $\Vert \bx - \dec(\argmin_{\bc_k} \Vert \enc(\bx) - \bc_k \Vert) \Vert$   & $\phi(\bx)$   & (various)                     & $(\bc_1, \ldots, \bc_K)$  & number of prototypes $K$                                      & \xmark & \cite{linde1980algorithm,gersho1992} \\
    \bottomrule
\end{tabular}
